SMaLL-100: Introducing Shallow Multilingual Machine Translation Model for Low-Resource Languages

In recent years, multilingual machine translation models have achieved promising performance on low-resource language pairs by sharing information between similar languages, thus enabling zero-shot translation. To overcome the "curse of multilinguality", these models often opt for scaling up the number of parameters, which makes their use in resource-constrained environments challenging. We introduce SMaLL-100, a distilled version of the M2M-100 (12B) model, a massively multilingual machine translation model covering 100 languages. We train SMaLL-100 with uniform sampling across all language pairs and therefore focus on preserving the performance of low-resource languages. We evaluate SMaLL-100 on different low-resource benchmarks: FLORES-101, Tatoeba, and TICO-19 and demonstrate that it outperforms previous massively multilingual models of comparable sizes (200-600M) while improving inference latency and memory usage. Additionally, our model achieves comparable results to M2M-100 (1.2B), while being 3.6x smaller and 4.3x faster at inference. Code and pre-trained models: https://github.com/alirezamshi/small100

==> KD M2M-100/abstract.tex <==
\begin{abstract}

In recent years,  multilingual machine translation models have achieved promising performance on low-resource language pairs by sharing information between similar languages, thus enabling zero-shot translation.  To overcome the "curse of multilinguality", these models often opt for scaling up the number of parameters, which makes their use in resource-constrained environments challenging. We introduce \textit{SMaLL-100}, a distilled version of the M2M-100~(12B) model, a massively multilingual machine translation model covering 100 languages. We train SMaLL-100 with uniform sampling across all language pairs and therefore focus on preserving the performance of low-resource languages.  We evaluate SMaLL-100 on different low-resource benchmarks: FLORES-101, Tatoeba, and TICO-19 and demonstrate that it outperforms previous massively multilingual models of comparable sizes (200-600M) while improving inference latency and memory usage. Additionally, our model achieves comparable results to M2M-100~(1.2B), while being 3.6$\times$ smaller and 4.3$\times$ faster at inference.\footnote{The code and pre-trained SMaLL-100 model is available at \url{https://github.com/alirezamshi/small100}.}


\end{abstract}


==> KD M2M-100/ack.tex <==
\section*{Acknowledgement}

The work is done during the research internship at NAVER LABS Europe. Alireza Mohammadshahi is supported by the Swiss National Science Foundation~(grant number CRSII5-180320).

==> KD M2M-100/conclusion.tex <==
\section{Conclusion}

We presented SMaLL-100 model, a shallow multilingual NMT model, focusing on low-resource languages. We evaluated our model on different NMT benchmarks.
SMaLL-100 significantly outperforms multilingual models of comparable size on all of the tested benchmarks (FLORES-101, Tatoeba, TICO-19) and is much faster at inference.
It also achieves competitive results with M2M-100 1.2B~\cite{m2m-100}, while being 4.3$\times$ faster at inference and 3.6$\times$ smaller. Compared to M2M-100~(12B), the biggest available MNMT model, SMaLL-100 loses nearly 1.7 spBLEU on average but it is significantly faster~(7.8$\times$) and smaller~(36$\times$), which makes it a good fit for resource-constrained settings. Additionally, we show that SMaLL-100 can achieve similar performance as M2M-100~(12B) with just a few steps of fine-tuning on specific language pairs.

==> KD M2M-100/implement.tex <==
\section{Experimental Setup}
\label{sec:setup}

\begin{table}
\centering
\begin{adjustbox}{width=0.7\linewidth}
\begin{tabular}{lc}

Resource Type & Criteria \\
\toprule
Very-Low & $|K| \leq 100K$  \\
Low & $100K < |K| \leq 1M $ \\
Medium & $1M < |K| \leq 100M $ \\
High & $100M < |K|$ \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{\label{tab:langdist} The criteria to split languages into different resource categories. $|K|$ is the amount of training data to/from English.}
\end{table}

\begin{table*}
	\begin{adjustbox}{width=\textwidth}
	\centering
	\begin{tabular}{lcc|cccccccccccc|c}\toprule
		 &\multicolumn{15}{c}{\hspace{2cm} Language Direction} \\
		\cmidrule{4-15} 
		Model & params & Speed & VL2VL & VL2L & VL2M & VL2H & L2VL & L2L & L2M & L2H & M2VL & M2L & H2VL & H2L & AVG \\ \midrule
		\textbf{FLORES-101} & & & &  &  &  & &  &  &  &  & &  & &  \\[0.1ex] 
		FLORES-124 & 175M & 5.3$\times$ & 3.3 & 3.4 & 6.0 & 7.8 & 3.7 & 3.1 & 6.9 & 8.8 & 6.9 & 5.2 & 8.1 & 6.0 & 5.8\\
		M2M-100 & 418M & 3.1$\times$ & 4.3 & 3.7 & 7.8 & 9.4 & 5.4 & 3.4 & 9.1 & 11.3 & 9.9 & 5.8 & 11.4 & 6.6 & 7.3 \\
		FLORES-124 & 615M & 2.9$\times$ & 5.1 & 5.1 & 9.2 & 11.2 & 5.8 & 4.7 & 10.6 & 13.1 & 10.3 & 7.6 & 11.5 & 8.5 & 8.6 \\
	    \textit{Finetuned-100} & 330M & 7.8$\times$ & 6.1 & 5.4 & 8.7 & 11.3 & 5.7 & 4.1 & 9.0 & 11.8 & 10.4 & 6.8 & 13.0 & 8.0 & 8.4 \\
	    \textit{SMaLL-100} & 330M & 7.8$\times$ & \underline{7.9} & \underline{7.0} & 10.3 & 12.6 & 8.4 & \underline{6.1} & 11.6 & 14.3 & \underline{13.7} & \underline{9.0} & \underline{16.7} & \underline{10.2} & \underline{10.7} \\
	    \midrule
	    M2M-100 & 1.2B & 1.8$\times$ & 6.7 & 6.1 & \underline{10.8} & \underline{12.8} & \underline{8.7} & \underline{6.1} & \underline{13.0} & \underline{15.9} & 13.6 & 8.8 & 15.4 & 9.7 & 10.6 \\
	    M2M-100 & 12B & 1$\times$ & \textbf{8.7} & \textbf{8.8} & \textbf{11.9} & \textbf{13.7} & \textbf{11.7} & \textbf{9.7} & \textbf{15.4} & \textbf{18.2} & \textbf{16.5} & \textbf{12.6} & \textbf{18.7} & \textbf{13.9} & \textbf{13.3} \\
          \midrule \midrule
	   \textbf{Tatoeba} & & & &  &  &  & &  &  &  &  & &  & &  \\[0.1ex] 
		FLORES-124 & 175M  & 5.3$\times$ & - &7.6 & 15.7 & 10.1 & 4.6 & 5.3 & 11.5 & 10.8 & 14.0 & 10.2 & 6.4 & 7.5 & 9.4 \\
		M2M-100 & 418M  & 3.1$\times$ &- & 7.4 & 19.7 & 12.3 & 5.9 & 5.3 & 13.8 & 13.2 & 14.9 & 11.7  & 7.7 & 9.0 & 10.9 \\
		FLORES-124 & 615M  & 2.9$\times$ & - & \textbf{9.1} & 19.4 & 11.4 & 6.9 & \underline{7.6} & 12.7 & 13.7 & 14.4 & 13.3 & 8.0 & 9.7  & 11.4 \\
	    \textit{Finetuned-100} & 330M  & 7.8$\times$ & - & 4.0 & 21.1 & \underline{14.4} & 7.7 & 5.2 & 15.3 & 14.2 & 14.0 & 12.1 & 8.9 & 8.3 & 11.4 \\
	    \textit{SMaLL-100} & 330M  & 7.8$\times$ & - & 4.6 & \underline{22.1} & \textbf{16.4} & \underline{8.7} & 7.0 & \underline{16.7} & 15.8 & 16.3 & \underline{14.5} & \underline{10.6} & \underline{11.2} & \underline{13.1} \\
	    \midrule
	    M2M-100 & 1.2B  & 1.8$\times$ &- & \underline{8.8} & 19.5 & 13.1 & \underline{8.7} & 7.2 & 16.3 & \underline{17.0} & \underline{17.2} & 13.4 & \textbf{10.7} & 11.1  & 13.0 \\
	    M2M-100 & 12B & 1$\times$ & - & 8.6 & \textbf{23.5} & 13.1 & \textbf{9.8} & \textbf{10.2} & \textbf{17.8} & \textbf{17.9} & \textbf{18.5} & \textbf{15.2} & \textbf{10.7} & \textbf{13.2} & \textbf{14.4} \\ \midrule \midrule
	    
	    
	    \textbf{TICO-19} & & & &  &  &  & &  &  &  &  & &  & &  \\[0.1ex] 
		FLORES-124 & 175M & 5.3$\times$ & 4.6 & 5.5 & 8.1 & 11.5 & 4.4 & 5.6 & 9.7& 12.2& 3.9& 8.0& 4.2& 8.7 & 7.2\\
		M2M-100 & 418M & 3.1$\times$ & 4.0 & 5.5 & 9.8 & 13.7 & 4.2 & 5.7 & 11.6 & 14.9 & 4.1 & 8.8 & 5.3 & 9.4 & 8.1 \\
		FLORES-124 & 615M & 2.9$\times$ &  4.6 & 7.4 & 11.5 & 16.4 & 4.8 & 7.6 & 12.9 & 16.7 & 4.4 & 10.7 & 4.4 & 11.5 & 9.4 \\
	    \textit{Finetuned-100} & 330M & 7.8$\times$ & 6.1 & 7.2 & 11.9 & 17.4 & 5.5 & 6.1 & 12.1 & 15.2 & \underline{6.4} & 9.0 & \underline{9.5} & 10.3 & 9.7 \\
	    \textit{SMaLL-100} & 330M & 7.8$\times$& \textbf{7.8} & \underline{8.8} & \underline{13.3} & \underline{19.0} & \textbf{8.0} & 8.5 & \underline{14.3} & 17.8 & \textbf{8.3} & \underline{11.5} & \textbf{11.3} & \underline{12.7} & \underline{11.8} \\ 
	    \midrule
	    M2M-100 & 1.2B & 1.8$\times$ & 5.4 & 8.2 & 13.2 & 18.9 & 6.0 & \underline{8.7} & 14.0 & \underline{19.2} & 5.2& \underline{11.5} & 6.1& 12.5 & 10.8 \\
	    M2M-100 & 12B & 1$\times$ & \underline{6.4} & \textbf{10.9} & \textbf{15.4} & \textbf{20.6} & \underline{7.8} & \textbf{11.9} & \textbf{16.6} & \textbf{21.4} & \underline{6.4} & \textbf{15.4} & 8.7& \textbf{16.4} & \textbf{13.1} \\
	    \midrule
		\bottomrule
	\end{tabular}
	\end{adjustbox} 
	\caption{\label{table:main} Average spBLEU performance on FLORES-101, Tatoeba, and TICO-19 benchmarks for different language pair categories, defined in Appendix~\ref{app:detail-eval}. FLORES-101 results are computed on language pairs where M2M-100 12B has spBLEU scores higher than 3 to avoid polluting the analysis with meaningless scores. The first and second columns give the model size and speed-up ratios compared to M2M-100~(12B). Last column is the average spBLEU performance over all mentioned language directions. The best scores are shown in bold, and the second best results are shown with underline.}
\end{table*}

\subsection{Evaluation Benchmarks}

\paragraph{FLORES-101} is a multilingual NMT benchmark, containing 3,001 sentences from different domains, that are derived from English Wikipedia. Sentences are translated into 101 languages by human translators~\cite{flores101}. It mostly includes low and medium-resource languages. We use {\tt devtest} subset for the evaluation.

\paragraph{Tatoeba} is a crowd-sourced collection of user-provided translations in different languages~\cite{tiedemann-2020-tatoeba}. We choose a subset of languages from {\tt test} set of Tatoeba Challenge,\footnote{\url{https://github.com/Helsinki-NLP/Tatoeba-Challenge}} which are covered by M2M-100. 

\paragraph{TICO-19} was created during the COVID-19 pandemic~\cite{anastasopoulos-etal-2020-tico}. It contains sentences from 36 languages in the medical domain, including 26 low-resource languages. We evaluate on languages which are covered by M2M-100~\cite{m2m-100}. 

Inspired by \citet{flores101}, we split the languages based on the amount of available training sentences aligned with English into 4 different categories: Very-Low~(VL), Low~(L), Medium~(M), and High-resource~(H). As the true amount of training data is both dependent on quality and quantity of parallel sentences, \citet{flores101} suggested to estimate it by computing the number of bitext data aligned with English, that is calculated from statistics of OPUS corpora~\cite{tiedemann-2012-parallel}. Table~\ref{tab:langdist} illustrates the criteria for choosing the category of different languages. More details about the distribution of language pair categories in each benchmark are provided in Appendix~\ref{app:detail-eval}. 

\subsection{Baselines}

\paragraph{M2M-100}\citet{m2m-100} is a recent many-to-many NMT model covering 100 languages. \citet{m2m-100} provide 3 variants with respectively 418M, 1.2B, and 12B parameters. We compare against these 3 variants.
\paragraph{FLORES-124} is an extension of M2M-100, covering additional 24 languages. Training data of the additional languages is derived from OPUS~\cite{tiedemann-2012-parallel}. \citet{flores101} provide two models with 175M and 615M parameters. We use both models as baselines. 
\paragraph{FineTuned-100} uses the same architecture as defined in Section~\ref{sec:method}, but KD loss~($\Lagr_{kd}$) is not used for training. For a fair comparison, it is trained for the same number of steps as SMaLL-100 model. 

\begin{table*}
\centering
\begin{adjustbox}{width=0.9\linewidth}
\begin{tabular}{lccccc}\toprule
    & &\multicolumn{3}{c}{Fine-tuned} \\
    \cmidrule{3-5} 
Language pair & Language Type & M2M-100 (418M) & SMaLL-100 & steps & M2M-100 (12B) \\ \midrule
Cebuano-English & Low & 18.6 & \textbf{29.8} & 0.5K & 27.7   \\
English-Igbo & Low & 9.2 & \textbf{15.7}  & 1.5K & 14.9 \\
English-Malayalam & Low & 16.7 & \textbf{20.8}  & 3K & 20.6 \\
Georgian-Russian & Medium & 6.9 & \textbf{13.1} & 0.5K & 10.1 \\
English-Italian & High & 33.3 & 33.4 & 20K & \textbf{33.5} \\
French-Italian & High & 31.3 & 31.5 & 20K & \textbf{32.0} \\
Italian-Spanish & High & 26.6 & 26.8 & 20K & \textbf{27.0} \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{\label{app:fine-tune} spBLEU performance of fine-tuned SMaLL-100 and M2M-100 (418M) for the specified step, and M2M-100~(12B) on FLORES-101 devtest. The "step" column is the number of training steps required to reach M2M-100~(12B) performance. The type of each language pair is defined as the minimum of source and target language categories.}
\end{table*}

\subsection{Implementation Details}

SMaLL-100 contains nearly 330M parameters with 12 encoder and 3 decoder Transformer layers.\footnote{It is initialized with M2M-100~(418M), using its first 3 decoder layers for the initialization of the student's decoder.} It is trained for 30 days on 16 TESLA V100-32GB GPUs,\footnote{4 GPUs are used for the training of the student model. 12 GPUs are utilized to do the model parallelism of the teacher model.} with a batch size of 1K tokens and accumulated gradients over 9 batches. We implement our model using fairseq repository.\footnote{\url{https://github.com/facebookresearch/fairseq}} We use {\tt last-checkpoint}\footnote{\url{https://github.com/facebookresearch/fairseq/tree/main/examples/m2m_100}} of M2M-100~(12B) for the teacher model. For decoding, the beam search of 5 is applied. All hyper-parameters regarding the architecture and optimization strategy are provided in Appendix~\ref{app:impl}. \\ 
For a faster convergence, we first fine-tune SMaLL-100 for 150k steps without distillation~($\Lagr_{kd}$). Then, it is trained with both losses for 756K steps~(nearly 1 epoch). For evaluation, we use SentencePiece BLEU~(spBLEU), as it is shown to be a fair metric in multilingual settings~\cite{flores101}.\footnote{It utilizes a SentencePiece tokenizer with 256K tokens:~\url{https://github.com/facebookresearch/flores}} We use the same tokenizer and dictionary as M2M-100.


==> KD M2M-100/intro.tex <==
\section{Introduction}

Neural Machine Translation~(NMT) systems are usually trained on datasets consisting of millions of parallel sentences, thus still performing poorly on low-resource languages, i.e., languages without a large amount of training data. 
Over the past few years, previous work has proposed several approaches to improve the quality of translations in low-resource languages, e.g., Multilingual Neural Machine Translation~(MNMT) models~\cite{johnson-etal-2017-googles,m2m-100,tang-etal-2021-multilingual,flores101}, back-translation~\cite{sennrich-etal-2016-improving,edunov-etal-2018-understanding} and unsupervised machine translation~\cite{garcia-etal-2021-harnessing,ko-etal-2021-adapting}. 
Massively MNMT models are particularly interesting for low-resource languages as they benefit the most from knowledge transfer from related languages~\cite{https://doi.org/10.48550/arxiv.1907.05019}. However, it is also seen that \textit{curse of multilinguality} hurts the performance of high-resource languages. So, previous work attempted to increase the model size to maintain the translation performance in both high and low-resource languages. This makes the use of these massively MNMT models challenging in real-world resource-constrained environments. To overcome this problem, we propose SMaLL-100, a \textbf{S}hallow \textbf{M}ultilingual M\textbf{a}chine Translation Model for \textbf{L}ow-Resource \textbf{L}anguages covering 100 languages, which is a distilled alternative of M2M-100~(12B)~\cite{m2m-100}, the most recent and biggest available multilingual NMT model. In this paper, we focus on very-low and low-resource language pairs as there is no reasonable-size universal model that achieves acceptable performance over a great number of low-resource languages. We do so by training SMaLL-100 on a perfectly balanced dataset.\footnote{All language pairs have the same sampling probability, regardless of their training data size.} While this leads to lower performance on the high-resource languages, we claim that this loss is easily recoverable through further fine-tuning.  We evaluate SMaLL-100 on different low-resource benchmarks, e.g., FLORES-101~\cite{flores101}, Tatoeba~\cite{tiedemann-2020-tatoeba}, and TICO-19~\cite{anastasopoulos-etal-2020-tico}. To summarize, our contributions are as follows:
\begin{itemize}[noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt]
\item We propose SMaLL-100, a shallow multilingual NMT model, focusing on low-resource language pairs.
\item We evaluate SMaLL-100 on several low-resource NMT benchmarks.
\item We show that our model significantly outperforms previous multilingual models of comparable size while being faster at inference. Additionally, it achieves comparable results with M2M-100~(1.2B) model, with 4.3$\times$ faster inference and a 3.6$\times$ smaller size.
\item While SMaLL-100 reaches 87.2\% performance of the 12B teacher model, we show that this gap can be closed with a few fine-tuning steps both for low and high-resource languages. 
\end{itemize}


==> KD M2M-100/limitations.tex <==
\section*{Limitations}

As mentioned in Section~\ref{sec:result}, SMaLL-100 model under-performs for some medium and high-resource languages, which could be resolved by further fine-tuning. Due to our computation constraint, we train SMaLL-100 model on nearly 6$\%$ of the original M2M-100 model. So, we encourage future research to increase the size of training data~(especially for low-resource languages) to achieve better performance. Also, future research could apply different distillation strategies~\cite{wu-etal-2020-skip,wang-etal-2021-selective}, as we just used word-level knowledge distillation loss~\cite{hu-etal-2018-attention}.

==> KD M2M-100/model.tex <==
\section{Model and Training}
\label{sec:method}
\newcommand{\Lagr}{\mathcal{L}}

\subsection{SMaLL-100 Architecture} 
It has been shown by \citet{kasai2021_deepshallow} that deep encoder / shallow decoder architectures can achieve good translation quality while being significantly faster at inference. \citet{berard-etal-2021-efficient} have confirmed that this is also valid for multilingual NMT. Here, we use a 12-layer Transformer encoder \cite{transformer} and 3-layer decoder. Table \ref{app:tab:hyper-params} in the Appendix \ref{app:impl} reports further details of the SMaLL-100 architecture. Different from M2M-100 model, we use language codes in the encoder side, as it is shown to perform better with shallow decoder architectures~\cite{berard-etal-2021-efficient}.  

\subsection{Training Strategy}
SMaLL-100 is trained with a combination of two loss functions: a standard Cross Entropy loss (CE) and a Knowledge Distillation loss (KD). Given source sequence $X$ and gold target translation $Y=(y_0,...,y_m)$, the CE loss is calculated as:
\begin{align}
\begin{split}
\Lagr_{ce} = - \sum_{j=0}^{m}\sum_{z=1}^{|K|} \mathbbm{1}\{y_j = z \} \operatorname{log}~p(y_j=z | y_{<j},X,\theta_S) 
\end{split}
\end{align}
where $|K|$ is the target vocabulary size, $\mathbbm{1}$ is the indicator function, and $\theta_S$ is the model parameters. $p()$ is the conditional probability function. \\
We additionally use a word-level distillation loss, which is the Kullback–Leibler divergence between the output distributions of the student and teacher models~\cite{hu-etal-2018-attention}. Specifically, it is calculated as:
\begin{align}
\begin{split}
\Lagr_{kd} = - \sum_{j=0}^{m}\sum_{z=1}^{|K|} q(y_j=z | y_{<j},X,\theta_T) \\
\times \operatorname{log}~p(y_j=z | y_{<j},X,\theta_S) 
\end{split}
\end{align}
where $\theta_T$ is parameters of the teacher model. $q()$ is the conditional probability of the teacher model. The total loss is computed as: 
\begin{align}
\begin{split}
\Lagr_{total} = \Lagr_{ce} + \alpha \Lagr_{kd}
\end{split}
\end{align}
where $\alpha$ is a trainable parameter. 

\subsection{Training Data} 
Our training data includes parallel sentences from CCMatrix~\cite{https://doi.org/10.48550/arxiv.1911.04944} and CCAligned~\cite{el-kishky-etal-2020-ccaligned} datasets, which are part of the training data used by \citet{m2m-100} to train the M2M-100 models. As our goal is to maintain the performance of low-resource languages, we balance the training data across all language pairs; specifically, 100K sentence pairs are sampled for each language pair.\footnote{For language pairs with less than 100K sentence pairs, we repeat their data. We randomly select 100K sentences for language pairs with more than 100K training sentences.} As a result, our training data contains nearly 456M parallel sentences, which is less than 6$\%$ of the original data on which M2M-100~\cite{m2m-100} was trained. We use the same languages as M2M-100.

==> KD M2M-100/relatedwork.tex <==
\section{Related Work}
\label{relatedwork}

\paragraph{Compression and Distillation.} Over the past few years, pre-trained models lead to significant improvement by increasing the parameter size~\cite{raffel2019exploring,m2m-100,zhang2022opt}, which makes it challenging to use them in the resource-constraint environment. Previous work use several compression techniques e.g. knowledge distillation~\cite{kim-rush-2016-sequence,light2021}, pruning~\cite{behnke-heafield-2020-losing,zhang-etal-2021-enlivening,mohammadshahi2022compressed}, and quantization~\cite{tao2022compression,yao2022zeroquant} to provide a reasonable-size model, while keeping the performance. 
\paragraph{Multilingual NMT.} It provides a single model to translate between any pair of languages, which significantly improves performance on low-resource languages thanks to knowledge transfer~\cite{haddow2021survey}. 
Several works~\cite{dong-etal-2015-multi,firat-etal-2016-multi,platanios-etal-2018-contextual,m2m-100,berard-etal-2021-efficient} propose to include both language-specific, and language-independent parameters in MNMT models. Recently, massively MNMT models~\cite{neubig-hu-2018-rapid,https://doi.org/10.48550/arxiv.1907.05019,aharoni-etal-2019-massively,m2m-100,zhang-etal-2020-improving} have been proposed to translate between more than 100 languages. However, these models usually contain a huge number of parameters to maintain performance in both high and low-resource languages. Different from the previous work, we introduce SMaLL-100, which outperforms previous models with comparable size in low-resource language directions, while achieving better speed and being smaller.


==> KD M2M-100/results.tex <==
\section{Results and Discussion}
\label{sec:result}

\subsection{Low-Resource NMT Benchmarks}

Table~\ref{table:main} shows the average spBLEU performance on FLORES-101, Tatoeba, and TICO-19 test sets for different categories of language directions.\footnote{Complete spBLEU calculations of different language pairs on tested NMT benchmarks are provided in Appendix~\ref{app:spbleu}. Speed is calculated on 2 TESLA V100-32GB GPUs with a batch size of 1 sentence over a subset of FLORES-101 devtest, containing nearly 10K sentences from all language pairs.} SMaLL-100 outperforms all the models with comparable sizes while being smaller and faster at inference. Specifically, it outperforms M2M-100 418M both in terms of performance (+3.1 spBLEU) and inference speed (2.5$\times$ faster). We believe that Finetuned-100 outperforms M2M-100 418M for low-resource languages thanks to finetuning on the balanced dataset.  The higher performance of SMaLL-100 compared to Finetuned-100 across all benchmarks shows the benefit of KD loss which allows to distill knowledge from the teacher model.  Additionally, SMaLL-100 achieves competitive results with M2M-100~(1.2B), while being 3.6$\times$ smaller and 4.3$\times$ faster at inference. Compared to the biggest M2M-100 model~(12B), SMaLL-100 loses nearly 1.7 spBLEU but is 36$\times$ smaller and 7.8$\times$ faster. Regarding medium and high-resource language pairs~(as shown in Appendix~\ref{app:spbleu:remain}), SMaLL-100 achieves better or similar performance compared to M2M-100~(418M) and FLORES-124~(615M), while it contains fewer parameters and is faster at the evaluation time. It under-performs for some medium and high-resource language pairs compared to the teacher model~(M2M-100 12B), which could be easily recovered, as we describe in the remaining section.

\subsection{Recovering Teacher Model Performance}
To go further, we demonstrate that SMaLL-100 can easily recover the performance of the teacher model with just a few fine-tuning steps, both for low and high-resource language pairs. For comparison, we fine-tune M2M-100 (418M) model with the same number of steps. \\
Table~\ref{app:fine-tune} reports spBLEU performance for several language pairs, alongside the number of fine-tuning steps, required by SMaLL-100 model to reach M2M-100 (12B) performance.\footnote{More dataset and implementation details of these fine-tuning experiments are provided in Appendix~\ref{app:detail-low}.}
We see that SMaLL-100 achieves better performance than M2M-100~(12B) after a few training steps on low-resource language pairs. For high-resource language pairs, SMaLL-100 is fine-tuned for 20K steps to reach the performance of M2M-100~(12B) model. Additionally, fine-tuned SMaLL-100 significantly outperforms fine-tuned M2M-100 (418M) model on low and medium-resource languages. This confirms that SMaLL-100 could be a powerful and lightweight initialization model for training on different language pairs.

